Multi-Attribute Selectivity Estimation Using Deep Learning

Selectivity estimation - the problem of estimating the result size of queries - is a fundamental problem in databases. Accurate estimation of query selectivity involving multiple correlated attributes is especially challenging. Poor cardinality estimates could result in the selection of bad plans by the query optimizer. We investigate the feasibility of using deep learning based approaches for both point and range queries and propose two complementary approaches. Our first approach considers selectivity as an unsupervised deep density estimation problem. We successfully introduce techniques from neural density estimation for this purpose. The key idea is to decompose the joint distribution into a set of tractable conditional probability distributions such that they satisfy the autoregressive property. Our second approach formulates selectivity estimation as a supervised deep learning problem that predicts the selectivity of a given query. We also introduce and address a number of practical challenges arising when adapting deep learning for relational data. These include query/data featurization, incorporating query workload information in a deep learning framework and the dynamic scenario where both data and workload queries could be updated. Our extensive experiments with a special emphasis on queries with a large number of predicates and/or small result sizes demonstrates that our proposed techniques provide fast and accurate selective estimates with minimal space overhead.

==> commands.tex <==
%!TEX root = main.tex
\newcommand{\eat}[1]{}

\usepackage{latexsym}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{xcolor}
\usepackage{colortbl}
\usepackage{epsfig}
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{paralist}
\usepackage{enumerate}
%\usepackage{enumitem}
%\usepackage[table]{xcolor}
%\usepackage[all]{xy}
\usepackage[color,matrix,arrow,all]{xy}
%\usepackage{cite}
\usepackage{comment}
\usepackage{booktabs}
\usepackage{balance}
\usepackage{stmaryrd}
\usepackage{pifont}
\usepackage{hhline}
%\usepackage{mathabx}
\usepackage{listings}
\usepackage{array}
\usepackage{float}
\usepackage[flushleft]{threeparttable}

\usepackage{wrapfig}

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT DELETE!!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{tikz}
%\usetikzlibrary{trees}

\usepackage{epsfig}
\usepackage{multirow}
\usepackage{url}

%\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage[export]{adjustbox}% http://ctan.org/pkg/adjustbox
\usepackage[noend]{algorithmic}
\usepackage{algorithm}

\newtheorem{myTheorem}{\textbf{Theorem}}
\newtheorem{myDefinition}{Definition}
\newtheorem{myExample}{\textbf{Example}}

%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
%\newcommand{\bform}{Boolean formula}
%\newcommand{\bForm}{Boolean Formula}
%\definecolor{orange}{HTML}{FF7F00}

\newcommand{\add}[1]{\textcolor{blue}{{#1}}}
\newcommand{\rewrite}[1]{\textcolor{gray}{{#1}}}
\newcommand{\notice}[1]{\textcolor{red}{{#1}}}

\newcommand{\eq}{\kw{eq}}

\newcommand{\ab}{\allowbreak}

\iffalse{%EAT
% eat by Nan, due to conflicts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Enumerate and Itemize modifications
%\usepackage{enumitem}
%\setlist{topsep=0pt,noitemsep}
%\setitemize[1]{label=$\circ$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
}\fi%EAT

\sloppy
\newcommand{\rtable}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\ratt}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\at}[1]{\protect\ensuremath{\mathsf{#1}}\xspace}
\newcommand{\myhrule}{\rule[.5pt]{\hsize}{.5pt}}
\newcommand{\oneurl}[1]{\texttt{#1}}
\newcommand{\tabstrut}{\rule{0pt}{4pt}\vspace{-0.1in}}
\newcommand{\stab}{\vspace{1.2ex}\noindent}
\newcommand{\sstab}{\rule{0pt}{8pt}\\[-2.2ex]}
\newcommand{\vs}{\vspace{1ex}}
\newcommand{\exa}[2]{{\tt\begin{tabbing}\hspace{#1}\=\+\kill #2\end{tabbing}}}
\newcommand{\ra}{\rightarrow}
\newcommand{\match}{\rightleftharpoons}

\newcommand{\true}{\kw{true}}
\newcommand{\kop}{\kw{op}}
\newcommand{\nil}{\kw{nil}}
\newcommand{\Op}{\kw{Op}}

\newcommand{\la}{\leftarrow}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\mat}[2]{{\begin{tabbing}\hspace{#1}\=\+\kill #2\end{tabbing}}}
\newcommand{\m}{\hspace{0.05in}}
\newcommand{\ls}{\hspace{0.1in}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\beqn}{\begin{eqnarray*}}
\newcommand{\eeqn}{\end{eqnarray*}}
\newcommand{\card}[1]{\mid\! #1\!\mid}
\newcommand{\fth}{\hfill $\Box$}
%\newcommand{\AND}{\displaystyle{\bigwedge_{i=1}^{n}}}
%\newcommand{\AND}{\displaystyle{\bigwedge_{i=1}^{m}}}
%\newcommand{\U}[1]{\displaystyle{\bigcup_{#1}}}
\newcommand{\Sm}[1]{\displaystyle{\sum_{#1}}}
\newcommand{\stitle}[1]{\vspace{1ex}\noindent{\bf #1}}
\newcommand{\ititle}[1]{\vspace{1ex}\noindent{\it #1}}
\newcommand{\etitle}[1]{\vspace{0.8ex}\noindent{\underline{\em #1}}}
\newcommand{\betitle}[1]{\vspace{0.8ex}\noindent{\underline{\bf {\em #1}}}}
\renewcommand{\t}{\tau}
\newcommand{\Inh}[1]{\$#1}
\renewcommand{\r}[1]{{\it rule}(#1)}
\newcommand{\pa}{\parallel}
\newcommand{\LHS}{\mbox{\small LHS}}
\newcommand{\RHS}{\mbox{\small RHS}}
\newcommand{\ie}{{\em i.e.,}\xspace}
\newcommand{\eg}{{\em e.g.,}\xspace}
\newcommand{\wrt}{\emph{w.r.t.}\xspace}
\newcommand{\aka}{\emph{a.k.a.}\xspace}
\newcommand{\kwlog}{\emph{w.l.o.g.}\xspace}
\newcommand{\Equa}{\mbox{\small EQU}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ALGORITHMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\SELECT}{\mbox{{\bf select}}\ }
\newcommand{\FROM}{\mbox{{\bf from}\ }}
\newcommand{\WHERE}{\mbox{\bf where}\ }
\newcommand{\SUM}{\mbox{{\bf sum}}\ }
\newcommand{\GROUPBY}{\mbox{{\bf group by}}\ }
\newcommand{\HAVING}{\mbox{{\bf having}}\ }
\newcommand{\CASE}{\mbox{{\bf case}}\ }
\newcommand{\END}{\mbox{{\bf end}}\ }
\newcommand{\WHEN}{\mbox{{\bf when}}\ }
\newcommand{\EXISTS}{\mbox{{\bf exists}}\ }
\newcommand{\COUNT}{\mbox{\kw{count}}}
\newcommand{\INSERTINTO}{\mbox{{\bf insert into}}\ }
\newcommand{\UPDATE}{\mbox{{\bf update}}\ }
\newcommand{\SET}{\mbox{{\bf set}}\ }
\newcommand{\IN}{\mbox{{\bf in}}\ }
\newcommand{\Null}{\mbox{{\it null}}}
%\newcommand{\If}{\mbox{\bf if}\ }
\newcommand{\Then}{\mbox{\bf then}\ }
\newcommand{\To}{\mbox{\bf to}\ }
\newcommand{\Let}{\mbox{\bf let}\ }
\newcommand{\Continue}{\mbox{\bf continue}\ }
%\newcommand{\Else}{\mbox{\bf else}\ }
%\newcommand{\ElseIf}{\mbox{\bf elseif}\ }
%\newcommand{\While}{\mbox{\bf while}\ }
%\newcommand{\Begin}{\mbox{\bf begin}\ }
%\newcommand{\End}{\mbox{\bf end}\ }
%\newcommand{\Do}{\mbox{\bf do}\ }
\newcommand{\Downto}{\mbox{\bf downto}\ }
%\newcommand{\Repeat}{\mbox{\bf repeat}\ }
\newcommand{\Until}{\mbox{\bf until}\ }
%\newcommand{\For}{\mbox{\bf for}\ }
%\newcommand{\ForEach}{\mbox{\bf for each}\ }
%\newcommand{\Or}{\mbox{\bf or}\ }
%\renewcommand{\And}{\mbox{\bf and}\ }
%\newcommand{\Not}{\mbox{\bf not}\ }
%\newcommand{\Return}{\mbox{\bf return}\ }
%\newcommand{\Case}{\mbox{\bf case}\ }
\newcommand{\Of}{\mbox{\bf of}\ }
\newcommand{\EndCase}{\mbox{\bf end-case}\ }
\newcommand{\NIL}{\mbox{\em nil}}
\newcommand{\False}{\mbox{\em false}}
\newcommand{\True}{\mbox{\em true}}
\newcommand{\algAND}{{\sc and}\xspace}
%\newcommand{\OR}{{\sc or}\xspace}
%\newcommand{\NOT}{{\sc not}\xspace}
\newcommand{\kw}[1]{{\ensuremath {\mathsf{#1}}}\xspace}
\newcommand{\cf}{\kw{cf}}

\newcounter{ccc}
\newcommand{\bcc}{\setcounter{ccc}{1}\theccc.}
\newcommand{\icc}{\addtocounter{ccc}{1}\theccc.}
\newcommand{\checking}{{\mbox{\small\sf Checking}\xspace}}
\newcommand{\fd}{\kw{fd}}
\newcommand{\preProcessing}{{\mbox{\small\sf preProcessing}\xspace}}
\newcommand{\CFDconsistency}{{\mbox{\small\sf CFD\_Checking}\xspace}}
\newcommand{\templateDB}{{\mbox{\small\sf templateDB}\xspace}}
\newcommand{\ChaseChecking}{{\mbox{\small\sf RandomChecking}\xspace}}
\newcommand{\chase}{{\mbox{\small\sf Chase}\xspace}}
\newcommand{\SAT}{{\mbox{\small\sf SAT}\xspace}}
\newcommand{\ECFD}{{\small eCFD}\xspace}
\newcommand{\DQR}{{\sc dqr}\xspace}
\newcommand{\MDM}{{\sc mdm}\xspace}
\newcommand{\CFD}{{\small CFD}\xspace}
\newcommand{\CFDs}{{\small CFDs}\xspace}
\newcommand{\DC}{{\small DC}\xspace}
\newcommand{\DCs}{{\small DCs}\xspace}

\newcommand{\ECFDs}{{\small eCFDs}\xspace}
\newcommand{\DQRs}{{\sc dqr}{\small s}\xspace}
\newcommand{\CIND}{{\sc cind}\xspace}
\newcommand{\MD}{{\small MD}\xspace}
\newcommand{\MDs}{{\small MDs}\xspace}
\newcommand{\cind}{{\small \sf CIND}}
\newcommand{\Damon}{\kw{Damon}}
\newcommand{\sol}{\kw{sol}}
\newcommand{\Rep}{\kw{Rep}}
\newcommand{\HFDs}{{\sc hfd}{\small s}\xspace}
\newcommand{\RCK}{{\sc rck}\xspace}
\newcommand{\RCKs}{{\sc rck}{\small s}\xspace}

\newcommand{\DRs}{{DRs}\xspace}
\newcommand{\DR}{{DR}\xspace}


\DeclareMathAlphabet{\pazocal}{OMS}{zplm}{m}{n}
\newcommand{\Us}{\pazocal{U}}




\newcommand{\FN}{\mbox{{\sc fn}}\xspace}
\newcommand{\SN}{\mbox{{\sc ln}}\xspace}
\newcommand{\LN}{\mbox{\sc ln}\xspace}
\newcommand{\post}{\at{post}}
\newcommand{\phn}{\at{phn}}
\newcommand{\kpost}{\at{post}}
\newcommand{\tel}{\at{tel}}
\newcommand{\addr}{\at{addr}}
\newcommand{\kemail}{\at{email}}

\newenvironment{tbi}{\begin{itemize}\vspace{0.5ex}
        \setlength{\topsep}{1ex}\setlength{\itemsep}{0.5ex}}
        {\end{itemize}}%\vspace{-0.5ex}}
\newenvironment{tbe}{\begin{enumerate}\vspace{0.5ex}
        \setlength{\topsep}{1ex}\setlength{\itemsep}{0.5ex}}
        {\end{enumerate}}%\vspace{-0.5ex}}

\newcommand{\wt}{\kw{wt}}
\newcommand{\cost}{\protect\ensuremath{\mathsf{cost}}\xspace}
\newcommand{\dis}{\protect\ensuremath{\mathsf{dis}}\xspace}
\newcommand{\repr}{D_r\xspace}

\newcommand{\CHFD}{{\sc chfd}\xspace}
\newcommand{\eHFD}{e{\sc hfd}\xspace}

\newcommand{\CHFDs}{{\sc chfd}{\small s}\xspace}
\newcommand{\eHFDs}{e{\sc hfd}{\small s}\xspace}
\newcommand{\kSN}{\kw{SN2}}
\newcommand{\FD}{{\small FD}\xspace}
\newcommand{\FDs}{{\small FD}{\small s}\xspace}
\newcommand{\IND}{{\sc ind}\xspace}
\newcommand{\INDs}{{\sc ind}{\small s}\xspace}
\newcommand{\TGDs}{{\sc tgd}{\small s}\xspace}
\newcommand{\NP}{{\small NP}\xspace}
\newcommand{\NC}{{\sc NC}\xspace}
\newcommand{\coNP}{co{\small NP}\xspace}
\newcommand{\PTIME}{{\sc PTIME}\xspace}
\newcommand{\PSPACE}{{\small PSPACE}\xspace}
\newcommand{\EXPTIME}{{\sc exptime}\xspace}
\newcommand{\NPSPACE}{{\sc npspace}\xspace}
\newcommand{\dom}{\protect\ensuremath{\mathsf{dom}}\xspace}
\newcommand{\adom}{\protect\ensuremath{\mathsf{adom}}\xspace}
\newcommand{\atset}{\protect\ensuremath{\mathsf{attr}}\xspace}
\newcommand{\attr}[1]{\protect\ensuremath{\mathsf{#1}}\xspace}
\newcommand{\attrset}{\protect\ensuremath{\mathsf{attr}}\xspace}
\newcommand{\finatset}{\protect\ensuremath{\mathsf{finattr}}\xspace}
\newcommand{\DNA}{{\sc dna}\xspace}
\newcommand{\PRATA}{{\sc prata}\xspace}
\newcommand{\XML}{{\sc xml}\xspace}
\newcommand{\RDF}{{\sc rdf}\xspace}
\newcommand{\KB}{{\sc kb}\xspace}
\newcommand{\KBs}{{\sc kb}{\small s}\xspace}
\newcommand{\URI}{{\sc uri}\xspace}
\newcommand{\URIs}{{\sc uri}{\small s}\xspace}
\newcommand{\HTML}{{\sc html}\xspace}
\newcommand{\UNIX}{{\sc unix}\xspace}
\newcommand{\DTD}{{\sc dtd}\xspace}
\newcommand{\JDBC}{{\sc jdbc}\xspace}
\newcommand{\DTDs}{{\sc dtd}{\small s}\xspace}
\newcommand{\SQL}{{\sc sql}\xspace}
\newcommand{\SQLU}{{\sc sqlu}\xspace}
\newcommand{\XSLT}{{\sc xslt}\xspace}
\newcommand{\DBMS}{{\sc dbms}\xspace}
\newcommand{\ATG}{{\sc atg}\xspace}
\newcommand{\ATGs}{{\sc atg}{\small s}\xspace}
\newcommand{\EBI}{{\sc ebi}\xspace}
\newcommand{\GO}{{\sc go}\xspace}
\newcommand{\VEC}[1]{{\sc vec}(#1)}
\newcommand{\DAG}{{\small DAG}\xspace}
\newcommand{\SCC}{{\small SCC}\xspace}
\newcommand{\SCCs}{{\small SCC}s\xspace}
\newcommand{\XQ}{{\sc xq}\xspace}
\newcommand{\XQwc}{{\sc xq}$^{\scriptscriptstyle[*]}$\xspace}
\newcommand{\XQdes}{{\sc xq}$^{\scriptscriptstyle[//]}$\xspace}
\newcommand{\XQfull}{{\sc xq}$^{\scriptscriptstyle[*,//]}$\xspace}
\newcommand{\SPARQL}{{\sc sparql}\xspace}
\newcommand{\vect}[1]{$\langle$ #1 $\rangle$}
\newcommand{\sem}[1]{[\![#1]\!]}
\newcommand{\NN}[2]{#1\sem{#2}}
\newcommand{\e}[2]{{\mathit (#1,#2)}}
\newcommand{\ep}[2]{{\mathit (#1,#2)+}}
\newcommand{\brname}{\ensuremath{{\mathsf{N}}}}
\newcommand{\budrel}[1]{\ensuremath{{\brname_{#1}}}}
\newcommand{\budgen}[2]{\ensuremath{Q^\brname_\e{#1}{#2}}}
\newcommand{\budcut}[2]{\ensuremath{Q_\e{#1}{#2}}}
\newcommand{\R}{{\cal R}}
%\newcommand{\G}{{\cal G}}
\newcommand{\I}{{\cal I}}
\newcommand{\V}{{\cal V}}
\newcommand{\E}{{\cal E}}
\newcommand{\eop}{\hspace*{\fill}\mbox{$\Box$}\vspace{1ex}}     % End of proof

%\newcounter{example}
%\renewcommand{\theexample}{\arabic{example}}
%\newenvironment{example}{
%        \vspace{1ex}
%        \refstepcounter{example}
%        {\noindent\bf Example \theexample:}}{
%        \eop}

\def\copyrightspace{}
\renewcommand{\ni}{\noindent}
\newcommand{\comlore}[1]{\begin{minipage}{3in}\fbox{\fbox{\parbox[t]{3in}{{\vspace{2mm}\noindent \bf COMM(LORE):~
{ #1}\hfill  END.}}}}\end{minipage}\\}
\newcommand{\comwenfei}[1]{\begin{minipage}{3in}\fbox{\fbox{\parbox[t]{3in}{{\vspace{2mm}\noindent \bf COMM(WENFEI):~
{ #1}\hfill  END.}}}}\end{minipage}\\}
\newcommand{\comshuai}[1]{\begin{minipage}{3in}\fbox{\fbox{\parbox[t]{3in}{{\vspace{2mm}\noindent \bf COMM(SHUAI):~
{ #1}\hfill  END.}}}}\end{minipage}\\}
\newcommand{\nthesection}{\arabic{section}}
%\newcounter{theorem}%[section]
%\renewcommand{\thetheorem}{\arabic{theorem}}
%\newcounter{prop}[section]
%\renewcommand{\theprop}{\nthesection.\arabic{theorem}}
%\newcounter{lemma}[section]
%\renewcommand{\thelemma}{\nthesection.\arabic{theorem}}
%\newcounter{cor}
%\renewcommand{\thecor}{\arabic{theorem}}
%\newenvironment{theorem}{\begin{em}
%        \refstepcounter{theorem}
%        {\vspace{1ex} \noindent\bf  Theorem  \thetheorem:}}{
%        \end{em}\eop} %\hspace*{\fill}\vspace*{1ex}}
%\newenvironment{prop}{\begin{em}
%        \refstepcounter{theorem}
%        {\vspace{1ex}\noindent \bf Proposition \thetheorem:}}{
%        \end{em}\eop}%\hspace*{\fill}\vspace*{1ex}}
%\newenvironment{lemma}{\begin{em}
%        \refstepcounter{theorem}
%        {\vspace{1ex}\noindent\bf Lemma \thelemma:}}{
%        \end{em}\eop} %\hspace*{\fill}\vspace*{1ex}}
%\newenvironment{cor}{\begin{em}
%        \refstepcounter{theorem}
%        {\vspace{1ex}\noindent\bf Corollary \thecor:}}{
%        \end{em}\eop} %\hspace*{\fill}\vspace*{1ex}}
%

%\newcounter{definition}[section]
%%\renewcommand{\thedefinition}{\nthesection.\arabic{definition}}
%\newcommand{\thedefinition}{\arabic{definition}}
%\newenvironment{definition}{
%        \vspace{1ex}
%        \refstepcounter{definition}
%        {\noindent\bf Definition {\bf \thedefinition}:}}{\eop
%}

\newenvironment{ctheorem}[1]{\begin{em}
        \refstepcounter{theorem}
        {\vspace{1ex}\noindent\bf  Theorem  {\bf \thetheorem} #1: }}{
        \end{em}\eop}

\newcounter{alg}[section]
\renewcommand{\thealg}{\nthesection.\arabic{alg}}
\newenvironment{alg}[1]{
        \refstepcounter{alg}
        {\vspace{1ex}\noindent\bf Algorithm \thealg:\, #1}}{
        \vspace*{1ex}}
\newcounter{arule}
\renewcommand{\thearule}{\arabic{arule}}
\newenvironment{arule}{
        \vspace{0.6ex}
        \refstepcounter{arule}
        {\noindent \em Rule \thearule:}}{
        }
\newcounter{claim}
\renewcommand{\theclaim}{\arabic{claim}}
\newenvironment{claim}{
        \vspace{0.6ex}
        \refstepcounter{claim}
        {\noindent\em Claim \theclaim:}}{
        }

%\newenvironment{proof}{
%        \vspace{0.5ex}
%        {\noindent\bf Proof:}}{\eop\vspace{1ex}}
\newenvironment{proofS}{
        \vspace{1ex}
        {\noindent\bf Proof sketch:\ }}{\eop\vspace{1ex}}

%\newcommand{\proofs}{\sstab{\bf Proof sketch.\ }\xspace}
\newcommand{\synthalg}{\textsc{RuleSynth}\xspace}
\newcommand{\algth}{\textsc{RS-BestTh}\xspace}
\newcommand{\algcompsyn}{\textsc{RS-SynthComp}\xspace}
\newcommand{\bestTh}{\textsc{BestThresholds}\xspace}
\newcommand{\compSyn}{\textsc{SynthComp}\xspace}

\newcommand{\Th}{\textbf{T}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\EG}{\mathbf{E}}
\newcommand{\DNF}{\mathbf{DNF}}
\newcommand{\GBF}{\mathbf{GBF}}

\newcommand{\gdnf}{G_\DNF}
\newcommand{\ggbf}{G_\GBF}
\newcommand{\gram}[1]{G_{#1}}
\newcommand{\erdnf}{\mathbf{ER}\text{-}\mathbf{GBF}}
\newcommand{\erform}{\mathbf{ER}\text{-}\mathbf{Formula}}
\newcommand{\ersyn}{\mathbf{ER}\text{-}\mathbf{Synth}}
\newcommand{\synth}{\textbf{Synth}}
\newcommand{\verify}{\textbf{Verify}}

\newcommand{\fsim}[1]{{\tt #1}}

\newcommand{\flev}{{\tt Levenstein}}
\newcommand{\fjac}{{\tt Jaccard}}
\newcommand{\feq}{{\tt Equal}}
\newcommand{\fcos}{{\tt Cosine}}
\newcommand{\fnonulls}{{\tt noNulls}}

\newcommand{\iR}{r}
\newcommand{\iC}{i}
\newcommand{\KR}{K_{\text{RANSAC}}}
\newcommand{\KC}{K_{\text{CEGIS}}}
\newcommand{\rPickCall}{\textbf{sample}}
\newcommand{\rPick}[1]{\rPickCall\left(#1\right)}
\newcommand{\Esyn}{\mathbf{E}_{\text{SYN}}}
\newcommand{\Constr}{\textit{constraints}}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\Ecex}{\overline{\EG}_{\dnf_{\iC}}}

\newcommand{\dnf}{\Phi}
\newcommand{\gbf}{\Phi}
\newcommand{\formula}{\Phi}
\newcommand{\met}{\mu}
\newcommand{\metF}{\met_{\text{F-measure}}}
\newcommand{\metP}{\met_{\text{precision}}}
\newcommand{\metR}{\met_{\text{recall}}}

\newcommand{\libsim}{\mathcal{F}}
\newcommand{\Sk}{\textsc{Sketch}~}
\newcommand{\sk}{\textsc{Sketch}}
\newcommand{\amopf}[3]{r[\at{A_#1}] {\approx}_{(#2,#3)} s[\at{A_#1'}]}
\newcommand{\amop}[1]{r[\at{A_#1}] {\approx} s[\at{A_#1'}]}
\newcommand{\amrule}[3]{{\approx}(#1,#2,#3)}
\newcommand{\amrulenew}[3]{\at{#2}[\at{#1}] \geq #3}
\newcommand{\ameqrule}[3]{{=}(#1,#2,#3)}
\newcommand{\fite}[3]{ \= \textbf{ if } \hspace{4ex} \= $#1$ \\ \> \textbf{ then } \> $#2$ \\ \> \textbf{ else } \> $#3$}
\newcommand{\fif}[2]{\textbf{if }#1\textbf{ then }#2}

\newcommand{\nfite}[3]{ \textbf{ if } $#1$ \textbf{ then } $#2$ \textbf{ else } $#3$}

%\newcommand{\ersyn}{\textrm{ErSyn}}

\newcommand{\MP}{matching pattern\xspace}
\newcommand{\MPs}{matching patterns\xspace}
\newcommand{\SP}{table pattern\xspace}
\newcommand{\SPs}{table patterns\xspace}

\newcommand{\algpd}{\textsc{PDiscovery}}
\newcommand{\algtval}{\textsc{CrowdTypeVal}}

\newcommand{\kb}{{\sc kb}\xspace}
\newcommand{\kbs}{{\sc kb}s\xspace}

\newcommand{\uk}{{\sc uk}\xspace}
\newcommand{\us}{{\sc us}\xspace}
\newcommand{\sys}{{\sc DeepER}\xspace}
\newcommand{\REP}{{\sc REP}\xspace}
\newcommand{\TRX}{{\sc TRX}\xspace}

%\newcommand{\system}{\textsc{Violet}\xspace}
\newcommand{\id}{\kw{id}}
\newcommand{\get}{{\sc get}}
\newcommand{\op}{\kw{op}}
\newcommand{\equ}{\kw{eq}}

\newcommand{\recall}{\kw{recall}}
\newcommand{\precision}{\kw{precision}}
\newcommand{\fmeasure}{\kw{F}-\kw{measure}}
\newcommand{\noi}{\kw{noi\%}}

\newcommand{\hosp}{{\sc hosp}\xspace}
\newcommand{\bus}{{\sc bus}\xspace}
\newcommand{\zip}{{\sc zip}\xspace}

\makeatletter
    \newcommand\figcaption{\def\@captype{figure}\caption}
    \newcommand\tabcaption{\def\@captype{table}\caption}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% FROM JIAN HE %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bluefont}[1]{{\color{blue} #1}}
\newcommand{\strong}[1]{ \textbf{\textit{#1}} }

\definecolor{shadecolor}{RGB}{200,200,200}
\newcommand{\mybox}[1]{\noindent\colorbox{shadecolor}
	{\parbox{\dimexpr\columnwidth-2\fboxsep\relax}{#1}}}
%{\vspace{1.5ex}\par\noindent\colorbox{shadecolor}
%	{\parbox{\dimexpr\columnwidth-2\fboxsep\relax}{#1}}\vspace{1.5ex}}


\definecolor{shadecolor1}{RGB}{230,230,230}
\newcommand{\myboxx}[1]{\par\noindent\colorbox{shadecolor1}
	{\parbox{\dimexpr\columnwidth-2\fboxsep\relax}{#1}}}

\definecolor{shadecolor1}{RGB}{255, 114, 118}
\newcommand{\tbd}[1]{\vspace{1ex}\par\noindent\colorbox{shadecolor1}
	{\parbox{\dimexpr\columnwidth-2\fboxsep\relax}{<== #1 ==>}}\vspace{1ex}}

	
\newcommand{\reminder}[1]{ {\mbox{$<==$}} [[[ \bluefont{ \bf #1 } ]]] {\mbox{$==>$}}}

\newcommand{\mycirc}[1][black]{\Large\textcolor{#1}{\ensuremath\bullet}}

%\newlength{\Oldarrayrulewidth}
%% Cline redefining to add line thickness
%\newcommand{\Cline}[2]{%
%  \noalign{\global\setlength{\Oldarrayrulewidth}{\arrayrulewidth}}%
%  \noalign{\global\setlength{\arrayrulewidth}{#1}}\cline{#2}%
%  \noalign{\global\setlength{\arrayrulewidth}{\Oldarrayrulewidth}}
%}


\newcommand{\nan}[1]{\footnote{\textcolor{blue}{Nan: #1}}}
\newcommand{\mourad}[1]{\footnote{\textcolor{blue}{Mourad: #1}}}
\newcommand{\sara}[1]{{\textcolor{blue}{Sara: #1}}}

\newcommand{\FDEq}[2]{#1 \rightarrow #2}


==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{Selectivity Estimation of Range Queries}
\label{subsec:rangePredicates}

Conjunctive queries with range constraints of the form $lb_i \leq A_i \leq ub_i$ are a popular class of queries for selectivity estimation
and has been extensively studied.
Given that our models produce accurate estimate of queries with equality constraints, 
a natural baseline is to exhaustively enumerate all distinct values between $lb_i$ and $ub_i$ and aggregate these point estimates.
If this interval is quite large then our proposed approaches can be easily extended to handle range queries.

\stitle{Supervised Estimation of Range Queries.}
The featurization process has to be modified to handle range predicates as a triplet $(A_i, lb_i, ub_i)$.
If attribute $A_i$ is unspecified, then $lb_i$ and $ub_i$ are set to the smallest and highest values respectively.
If the range query is one sided where either $lb_i$ or $ub_i$ is specified, the other is automatically set to the smallest/highest value as appropriate.
As before, the values of $lb_i$ and $ub_i$ must be normalized between an interval of $[0,1]$ using min-max scaling 
such that the smallest value of $A_i$ is represented as $0$ while highest value is set as $1$.
We used MHIST~\cite{poosala1997selectivity} heuristic to identify optimal cut-off points for individual attributes.
This is used for enumerating all possible range queries for generating queries with 1 predicate for training.
Suppose that the domain of attribute $A_1$ is partitioned as $[v_{11}, v_{12}, \ldots,]$. 
Then we generate all possible 1-predicate queries $\{v_{11} \leq A_1 \leq v_{12}\}, \{v_{11} \leq A_1 \leq v_{13}\}, \ldots, \{v_{12} \leq A_1 \leq v_{13}\}, \{v_{12} \leq A_1 \leq v_{14}\}, \ldots$ etc.
We then generate all possible 2-predicate queries as a cartesian product of 1-predicate range queries of two attributes and so on.
For arbitrary number of predicates, we modify our approach to \emph{randomly pick an interval} for chosen attribute $A_i$. 

\stitle{Unsupervised Estimation of Range Queries.}
Similar to the supervised learning approach, we begin by discretizing each individual attributes into multiple buckets through the MHIST heuristic~\cite{poosala1997selectivity}.
Each bucket $B$ for attribute $A_i$ is specified by the interval $[B_l, B_u]$. 
We then train our MADE based model on this discretized set of tuples.
Given a new query $lb_i \leq A_i \leq ub_i$, we identify all buckets $B$ for which the range $[B_l, B_u]$ overlap. 
For each bucket $B$ that is completely subsumed by the range, we use MADE to obtain the estimate and add them up. 
If a bucket $B$ partially overlaps with the query range, then we need to approximate the frequency that falls in this range.
%Improved Histograms for Selectivity Estimation of Range Predicates
For this, we use the uniform spread assumption proposed in~\cite{poosala1996improved} that states that 
each attribute value within a bucket has a spread equal to the bucket average.
This could be easily achieved by augmenting each bucket with the number of distinct values in it (in addition to $B_l$ and $B_u$).
Please refer to~\cite{poosala1996improved} for further details.

\subsection{Practical Issues}
\label{subsec:practicalIssues}

\stitle{Handling Attributes with Large Domain Sizes.}
A fundamental challenge in selectivity estimation is handling attributes with large domain sizes.
For numerical attributes, one can use heuristics such as V-Optimal~\cite{poosala1996improved} for discretization into a small number of buckets.
Handling categorical attributes is much trickier.
Blindly using the entire domain might cause the one-hot encoding to explode.
This has the spill on effect of increasing the model size and thereby the training time.
%Arguments end of Sec 2 of Daphne's paper.
There are two common approaches to partially ameliorate this issue.
First, when available one could leverage feature hierarchies~\cite{han2011data} to reduce the domain size and instead operate at the hierarchy level.
Alternatively, one could use clustering based techniques on categorical data that seek to minimize the entropy of the clusters~\cite{han2011data}.
Each value in the cluster is then represented through the cluster id. 

\stitle{Injecting Domain Knowledge.}
There are many ways to inject domain knowledge to improve the estimation accuracy.
We briefly mention few ideas.
\begin{itemize}
	\item One could preferentially bias the supervised model to estimate the selectivities of certain attribute combinations more accurately. 
		This could be easily achieved by increasing their corresponding weights in the query log.
		The model would be penalized more heavily for incorrect estimates for queries involving these attribute combinations.
		This will force the model to modify its weights so as to generate the estimates more accurately. 
	\item One could handle the order sensitivity of MADE by carefully selecting how the permutations are chosen.
		If a domain expert knows that variables $A_i$ and $A_j$ are order sensitive, then we only chose permutations where the desired order is observed.
		As a concrete example, if one knows (say via data profiling), that a functional dependency $A_i \rightarrow A_j$ exists.
		Then we would prefer permutations where $A_j$ has a higher index than $A_i$. 
	\item By default, our supervised and unsupervised models use Cross Entropy (CE) and Mean Squared Loss (MSE) as the loss functions.
		It is possible to modify our models to directly minimize selectivity estimation errors such as mean of q-errors or relative error. 
		As long as the metric is continuous and differentiable, the automatic differentiation techniques in most popular DL frameworks can handle them transparently.
		In our experiments, we did not find any major improvement by using these custom error functions.
		Hence, we sticked with the well known CE and MSE.
\end{itemize}

\stitle{Estimating Join Selectivities.}
One of the major attractions of DL based approaches is their effectiveness in handling correlated attributes.
Estimating the selectivities of correlated joins is especially challenging
with most state of the art approaches generating systematic and large under-estimations~\cite{leis2015good}.
An intuitive approach for applying our work for estimating join selectivities 
is to obtain a uniform random sample of the joins using any prior work on join sampling~\cite{chaudhuri1999random,leis2017cardinality} and train the MADE model on it.
As we shall show later in the experiments, this achieves promising results for individual joins 
even though our approaches are not explicitly designed for join estimations. 
The performance deteriorates as the number of relations that are being joined increases.
Extending neural density estimation techniques for join selectivities is a promising avenue for future work. 
For example, our MADE based approach could be easily used as a black box estimator for individual tables 
%cite: index sampling and learned cardinalities
inside state-of-the-art join estimation approaches such as ~\cite{leis2017cardinality}.

%\subsection{Neural and Non-Neural Selectivity Estimation}
%\label{subsec:neuralNonNeuralSelectivityEstimation}
%Intuitively, the traditional sampling and synopses approaches can be considered as approximate non-parameteric density estimators.
%In this work, we introduced a specific class of DL methods based on masked autoencoders for selectivity estimation.
%This approach is simple, expressive, efficient to train and well suited for database selectivity problems.
%We now briefly compare and contrast  DL based selectivity estimators with traditional estimators.

%Histograms are a powerful and popular tool for selectivity estimation.
%For small number of dimensions, they are compact, reasonably accurate and easy to maintain.
%However, their efficacy begins to degenerate for higher dimensions.
%Due to the curse of dimensionality, multi-dimensional histograms either require 
%lot of space for meaningful accuracy or have to resort to simplifications such as attribute value independence.
%DL based methods allow more complex ways to partition the probability density 
%and can leverage parametric densities and latent representations via autoencoders.
%Recall from Section~\ref{sec:unsupervised} that MADE could use Bernoulli distribution for categorical data 
%and (mixture of) Gaussians for numeric data.
%This straddling of parametric and non-parametric approaches give lot of power to 

%\red{Dr.Das comments.}

